Deep Sinogram Completion with Image Prior for Metal Artifact Reduction in CT Images

Computed tomography (CT) has been widely used for medical diagnosis, assessment, and therapy planning and guidance. In reality, CT images may be affected adversely in the presence of metallic objects, which could lead to severe metal artifacts and influence clinical diagnosis or dose calculation in radiation therapy. In this paper, we propose a generalizable framework for metal artifact reduction (MAR) by simultaneously leveraging the advantages of image domain and sinogram domain-based MAR techniques. We formulate our framework as a sinogram completion problem and train a neural network (SinoNet) to restore the metal-affected projections. To improve the continuity of the completed projections at the boundary of metal trace and thus alleviate new artifacts in the reconstructed CT images, we train another neural network (PriorNet) to generate a good prior image to guide sinogram learning, and further design a novel residual sinogram learning strategy to effectively utilize the prior image information for better sinogram completion. The two networks are jointly trained in an end-to-end fashion with a differentiable forward projection (FP) operation so that the prior image generation and deep sinogram completion procedures can benefit from each other. Finally, the artifact-reduced CT images are reconstructed using the filtered backward projection (FBP) from the completed sinogram. Extensive experiments on simulated and real artifacts data demonstrate that our method produces superior artifact-reduced results while preserving the anatomical structures and outperforms other MAR methods.

==> related.tex <==
\section{Related Work}
\label{sec:relatedwork}

\subsection{Conventional Metal Artifact Reduction}
Metal artifact reduction is a long-standing problem in image reconstruction field. 
The previous metal artifact reduction approaches mainly address this problem  in X-ray projections (sinogram). 
%
The metal-affected regions in sinogram are corrected by modeling the underlying physical effects of imaging~\cite{hsieh2000iterative,kachelriess2001generalized,meyer2010empirical,park2015metal}.
For example, Park \etal~\cite{park2015metal}  proposed a new method to correct beam hardening artifacts caused by the presence of metal in polychromatic X-ray CT. 
%
However, the metal trace regions in sinogram are often severe corrupted and the above methods cannot achieve satisfactory results. 
%%
Therefore, the widely used MAR methods regard the metal-affected regions as missing and replace them with estimated values~\cite{kalender1987reduction,mehranian2013x}.
%
The early Linear interpolation (LI) approach~\cite{kalender1987reduction} filled the missing data by the linear interpolation of its neighboring unaffected data for each projection view, while it often introduces new artifacts near large metals, as interpolation cannot completely recover the metal trace information.
%
Meyer \etal~\cite{meyer2010normalized} improved the LI approach by generating a prior image with tissue processing and normalizing the projection with the forward projection of the prior image before interpolation.
 %%
Besides interpolation in projection (sinogram) domain, there are also some works focusing on designing new iterative reconstruction algorithms to construct artifact-free images from the unaffected or corrected projections~\cite{wang1996iterative,wang1999iterative,lemmens2008suppression,zhang2011metal}.
%%
\ylq{For example, XXX}
However, these iterative reconstruction methods often suffer from a large amount of computation and require proper hand-crafted regularizations. 

\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figure/framework2.pdf}
	\caption{Schematic diagram of our proposed self-supervised joint learning framework for metal artifact reduction. We jointly train a sinogram completion network, \ie, SinoNet and an image refinement network, \ie, ImageNet. 
		In the testing phase (b), we use the forward projection of CNN output as prior sinogram to replace the metal-affected values in original sinogram, and the metal-free image is reconstructed from corrected sinogram with FBP algorithm.}
	\label{fig:network_arch}
	\centering
	\vspace{-0.5cm}
\end{figure*}


\subsection{Deep Learning Based Methods for MAR}
Plenty of deep learning methods have recently been proposed to conduct MAR in sinogram domain, image domain and jointly in two domains.
%%
Park~\etal employed a U-Net~\cite{ronneberger2015u} to correct metal-induced beam hardening in the projection domain~\cite{park2018ct} and image domain~\cite{park2017machine}, respectively, while 
Gjesteby~\etal developed a few deep learning based MAR methods that refine the performance of  NMAR, with deep learning in the projection domain~\cite{gjesteby2017deep} and image domain~\cite{gjesteby2017reducing,gjesteby2017deep}, respectively.
%
The CNN was used to help overcome residual errors from the NMAR. While their experiments demonstrated that CNN can improve the NMAR effectively, remaining artifacts are still considerable.
%%
More recently,  RL-ARCNN~\cite{huang2018metal} introduced residual learning into a deep convolutional neural network (CNN) and achieved better MAR performance than standard CNN. 
%
Gjesteby~\cite{gjesteby2018deep} employed a deep network to reduce
the secondary artifacts after the normalized MAR method with a perceptual loss.
% 
CNNMAR~\cite{zhang2018convolutional} uses CNN to generate prior images in the CT image domain to help the correction in the projection domain. Both DestreakNet and CNNMAR show significant improvements over the existing non-DNN based methods on synthesized datasets. cGANMAR~\cite{wang2018conditional} leverages generative adversarial networks (GANs) [13] to further improve the DNN- based MAR performance.
%%
There are also some works to utilize dual domain learning~\cite{lin2019dudonet,lyu2020dudonet}.
%%
 
